CACTUS: A depleted monolithic active timing sensor using a CMOS radiation hard technology

The planned luminosity increase at the Large Hadron Collider in the coming years has triggered interest in the use of the particles' time of arrival as additional information in specialized detectors to mitigate the impact of pile-up. The required time resolution is of the order of tens of picoseconds, with a spatial granularity of the order of 1 mm. A time measurement at this precision level will also be of interest beyond the LHC and beyond high energy particle physics. We present in this paper the first developments towards a radiation hard Depleted Monolithic Active Pixel Sensor (DMAPS), with high-resolution time measurement capability. The technology chosen is a standard high voltage CMOS process, in conjunction with a high resistivity detector material, which has already proven to efficiently detect particles in tracking applications after several hundred of Mrad of irradiation.

==> tex/OLD-biblio.tex <==
\bibitem{Allaire1}
C. Allaire et al., \emph{Beam test measurements of Low Gain Avalanche Detector single pads and arrays for the ATLAS High Granularity Timing Detector}, \emph{JINST} {\bf 13} (2018).

\bibitem{Pieric1}
I. Peric, \emph{A novel monolithic pixelated particle detector implemented in high-voltage CMOS technology}, \emph{Nucl. Instrum. Meth. A} {\bf 582} (2007) 876.

\bibitem{Chen1}
Z. Chen et al., \emph{Test results of irradiated CMOS pixel circuits in 150 nm CMOS technology for the ATLAS Inner Tracker Upgrade,} PoS (TWEPP 2018) 343.

\bibitem{Barbero1}
M. Barbero et al., \emph{Radiation hard DMAPS pixel sensors in 150nm CMOS technology for operation at LHC}, submitted in \emph{JINST} (2019), available on arXiv:1911.01119.

\bibitem{Iacobucci1}
G. Iacobucci1 et al., \emph{A 50 ps resolution monolithic active pixel sensor without internal gain in SiGe BiCMOS technology}, \emph{JINST} {\bf 19} (2019).

\bibitem{Degerli1}
Y. Degerli et al., \emph{Pixel architectures in a HV-CMOS process for the ATLAS inner detector upgrade}, \emph{JINST} {\bf 11} (2016).

\bibitem{Degerli2}
Y. Degerli et al., \emph{Characterization of an new HV/HR CMOS sensor in LF150nm process for the ATLAS inner tracker upgrade,} IEEE NSS Conf. Rec., 21-28 Oct. 2017, Atlanta, GA, USA.

\bibitem{Wang1}
T. Wang et al., \emph{Development of a depleted monolithic CMOS sensor in a 150 nm CMOS technology for the ATLAS inner tracker upgrade}, \emph{JINST} {\bf 12} (2017).

\bibitem{Synopsys}
Synopsys, Synopsys TCAD, \emph{https://www.synopsys.com/silicon/tcad.html}.

\bibitem{Guilloux1}
F. Guilloux et al., \emph{CACTUS: High-voltage CMOS monolithic active pixel sensor for tracking and time tagging of charged particles,} PoS (TWEPP 2017) 023.

\bibitem{Caicedo1}
I. Caicedo et al., \emph{The Monopix chips: depleted monolithic active pixel
sensors with a column-drain read-out architecture for the
ATLAS Inner Tracker upgrade}, \emph{JINST} {\bf 14}, (2019).

\bibitem{Mendic1}
I. Mandic et al., \emph{Neutron irradiation test of depleted CMOS pixel detector prototypes}, \emph{JINST} {\bf 12}, (2017).

\bibitem{FTBF}
"Fermilab Test Beam Facility," [Online]. Available: https://ftbf.fnal.gov. 
